TopicRNN: A Recurrent Neural Network with Long-Range Semantic Dependency

In this paper, we propose TopicRNN, a recurrent neural network (RNN)-based language model designed to directly capture the global semantic meaning relating words in a document via latent topics. Because of their sequential nature, RNNs are good at capturing the local structure of a word sequence - both semantic and syntactic - but might face difficulty remembering long-range dependencies. Intuitively, these long-range dependencies are of semantic nature. In contrast, latent topic models are able to capture the global underlying semantic structure of a document but do not account for word ordering. The proposed TopicRNN model integrates the merits of RNNs and latent topic models: it captures local (syntactic) dependencies using an RNN and global (semantic) dependencies using latent topics. Unlike previous work on contextual RNN language modeling, our model is learned end-to-end. Empirical results on word prediction show that TopicRNN outperforms existing contextual RNN baselines. In addition, TopicRNN can be used as an unsupervised feature extractor for documents. We do this for sentiment analysis on the IMDB movie review dataset and report an error rate of $6.28\%$. This is comparable to the state-of-the-art $5.91\%$ resulting from a semi-supervised approach. Finally, TopicRNN also yields sensible topics, making it a useful alternative to document models such as latent Dirichlet allocation.

==> preamble.tex <==
% # FONTS

\usepackage[T1]{fontenc}
\usepackage{tgtermes}

% NOTE: MUST INSTALL SEPARATELY
%\usepackage[subscriptcorrection,
%           amssymbols,
%           mtpbb,
%           mtpcal,
%           nofontinfo  % suppresses all warnings
%          ]{mtpro2}

% NOTE: MUST UNCOMMENT IF NOT USING MTPRO2
% \usepackage{amssymb}
% \newcommand{\mathbold}[1]{\ensuremath{\boldsymbol{\mathbf{#1}}}}

\usepackage{scalefnt,letltxmacro}
\LetLtxMacro{\oldtextsc}{\textsc}
\renewcommand{\textsc}[1]{\oldtextsc{\scalefont{1.10}#1}}
% \renewcommand*\ttdefault{lmvtt}
%\usepackage[ttdefault=true]{AnonymousPro}

% # MATH

\usepackage{amsmath, amsthm, amsfonts}
\usepackage{mathtools}

% # SPACING and TEXT

\usepackage[
  paper  = letterpaper,
  left   = 1.50in,
  right  = 1.50in,
  top    = 1.0in,
  bottom = 1.0in,
  ]{geometry}
% \usepackage[final,expansion=alltext]{microtype}
\usepackage[english]{babel}
\usepackage[parfill]{parskip}
\usepackage{afterpage}
\usepackage{enumitem}
\usepackage{framed}
\usepackage{xspace}

% # EDITING

\usepackage{lineno}
\renewcommand\linenumberfont{\normalfont
                             \footnotesize
                             \sffamily
                             \color{SkyBlue}}

\usepackage{ragged2e}
\DeclareRobustCommand{\sidenote}[1]{\marginpar{
                                    \RaggedRight
                                    \textcolor{Plum}{\textsf{#1}}}}

\newcommand{\parnum}{\bfseries\P\arabic{parcount}}
\newcounter{parcount}
\newcommand\p{%
    \stepcounter{parcount}%
    \leavevmode\marginpar[\hfill\parnum]{\parnum}%
}
\DeclareRobustCommand{\parhead}[1]{\textbf{#1}~}

% # COLOR

\usepackage[usenames,dvipsnames]{xcolor}
\definecolor{shadecolor}{gray}{0.9}

\newcommand{\red}[1]{\textcolor{BrickRed}{#1}}
\newcommand{\orange}[1]{\textcolor{BurntOrange}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{MidnightBlue}{#1}}
\newcommand{\sky}[1]{\textcolor{SkyBlue}{#1}}
\newcommand{\gray}[1]{\textcolor{black!60}{#1}}

% # COUNTERS

\renewcommand{\labelenumi}{\color{black!67}{\arabic{enumi}.}}
\renewcommand{\labelenumii}{{\color{black!67}(\alph{enumii})}}
\renewcommand{\labelitemi}{{\color{black!67}\textbullet}}

% # FIGURES

\usepackage{graphicx}
\usepackage[labelfont=bf]{caption}
\usepackage[format=hang]{subcaption}

% # TABLES

\usepackage{booktabs, array}

% # ALGORITHMS

% # BIBLIOGRAPHY AND LINKS

\usepackage{natbib}
\usepackage[algoruled]{algorithm2e}
\setlength{\interspacetitleruled}{8pt}
\usepackage{listings}
\usepackage{fancyvrb}
\fvset{fontsize=\small}
\usepackage[colorlinks,linktoc=all]{hyperref}
\usepackage[all]{hypcap}
\hypersetup{citecolor=MidnightBlue}
\hypersetup{linkcolor=MidnightBlue}
\hypersetup{urlcolor=MidnightBlue}
\usepackage[nameinlink, poorman]{cleveref}
\creflabelformat{equation}{#2\textup{#1}#3}  % <- remove parenthesis from equations

% # ACRONYMS

\usepackage
[acronym,smallcaps,nowarn,section,nonumberlist]{glossaries}
\glsdisablehyper{}
% \usepackage{glossary-mcols}
%\setglossarystyle{long3col}
%\setlength\glsdescwidth{0.8\linewidth}
%\setlength\glspagelistwidth{0pt}
%\makeglossaries

% # CODE SNIPPETS

\lstdefinestyle{mystyle}{
    commentstyle=\color{OliveGreen},
    numberstyle=\tiny\color{black!60},
    stringstyle=\color{BrickRed},
    basicstyle=\ttfamily\scriptsize,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=none,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}
\lstset{style=mystyle}

% # USEFUL COMMANDS

\newcommand{\pp}{\textcolor{Plum}{\P\,}}
\newcommand{\q}[1]{\red{{\sf Q | #1}}}
\newcommand{\draftdisclaimer}{\begin{center}\begin{framed} DRAFT: DO
NOT CITE OR DISTRIBUTE \end{framed}\end{center}}
\newcommand{\note}[2]{\red{\textsc{#1} | \textsf{#2}}}

% # SECTIONS AND TITLES

\RequirePackage[bf,small]{titlesec}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "lm"
%%% End:

==> preamble_acronyms.tex <==
\newacronym{ELBO}{elbo}{Evidence Lower Bound}
\newacronym{VI}{vi}{variational inference}
\newacronym{KL}{kl}{Kullback-Leibler}
\newacronym{RNN}{rnn}{recurrent neural network}
\newacronym{RNNs}{rnns}{recurrent neural networks}
\newacronym{RNNLM}{rnnlm}{Recurrent Neural Network-based language model}
\newacronym{TopicRNN}{TopicRNN}{TopicRNN}
\newacronym{TopicLSTM}{TopicLSTM}{TopicLSTM}
\newacronym{TopicGRU}{TopicGRU}{TopicGRU}
\newacronym{LSTM}{LSTM}{LSTM}
\newacronym{GRU}{GRU}{GRU}
\newacronym{IMDB}{IMDB}{IMDB}


==> preamble_math.tex <==
% # PROBABILITY

\newcommand{\g}{\,|\,}
\renewcommand{\gg}{\,\|\,}
\DeclareRobustCommand{\KL}[2]{\ensuremath{\textrm{KL}\left(#1\;\|\;#2\right)}}
\newcommand{\ind}{\mathbb{1}}

% # DISTRIBUTIONS

\newcommand{\Gam}{\textrm{Gam}}
\newcommand{\InvGam}{\textrm{InvGam}}

% # MISCELLANEOUS

\renewcommand{\d}[1]{\ensuremath{\operatorname{d}\!{#1}}}
\newcommand{\diag}{\textrm{diag}}
\newcommand{\supp}{\textrm{supp}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\E}[1]{\mathbb{E}\left[ #1 \right]}
\newcommand{\EE}[2]{\mathbb{E}_{#1}\left[ #2 \right]}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\rep}{\textrm{rep}}

% # BOLD MATHEMATICS

\newcommand{\mba}{\mathbold{a}}
\newcommand{\mbb}{\mathbold{b}}
\newcommand{\mbc}{\mathbold{c}}
\newcommand{\mbd}{\mathbold{d}}
\newcommand{\mbe}{\mathbold{e}}
%\newcommand{\mbf}{\mathbold{f}}
\newcommand{\mbg}{\mathbold{g}}
\newcommand{\mbh}{\mathbold{h}}
\newcommand{\mbi}{\mathbold{i}}
\newcommand{\mbj}{\mathbold{j}}
\newcommand{\mbk}{\mathbold{k}}
\newcommand{\mbl}{\mathbold{l}}
\newcommand{\mbm}{\mathbold{m}}
\newcommand{\mbn}{\mathbold{n}}
\newcommand{\mbo}{\mathbold{o}}
\newcommand{\mbp}{\mathbold{p}}
\newcommand{\mbq}{\mathbold{q}}
\newcommand{\mbr}{\mathbold{r}}
\newcommand{\mbs}{\mathbold{s}}
\newcommand{\mbt}{\mathbold{t}}
\newcommand{\mbu}{\mathbold{u}}
\newcommand{\mbv}{\mathbold{v}}
\newcommand{\mbw}{\mathbold{w}}
\newcommand{\mbx}{\mathbold{x}}
\newcommand{\mby}{\mathbold{y}}
\newcommand{\mbz}{\mathbold{z}}

\newcommand{\mbA}{\mathbold{A}}
\newcommand{\mbB}{\mathbold{B}}
\newcommand{\mbC}{\mathbold{C}}
\newcommand{\mbD}{\mathbold{D}}
\newcommand{\mbE}{\mathbold{E}}
\newcommand{\mbF}{\mathbold{F}}
\newcommand{\mbG}{\mathbold{G}}
\newcommand{\mbH}{\mathbold{H}}
\newcommand{\mbI}{\mathbold{I}}
\newcommand{\mbJ}{\mathbold{J}}
\newcommand{\mbK}{\mathbold{K}}
\newcommand{\mbL}{\mathbold{L}}
\newcommand{\mbM}{\mathbold{M}}
\newcommand{\mbN}{\mathbold{N}}
\newcommand{\mbO}{\mathbold{O}}
\newcommand{\mbP}{\mathbold{P}}
\newcommand{\mbQ}{\mathbold{Q}}
\newcommand{\mbR}{\mathbold{R}}
\newcommand{\mbS}{\mathbold{S}}
\newcommand{\mbT}{\mathbold{T}}
\newcommand{\mbU}{\mathbold{U}}
\newcommand{\mbV}{\mathbold{V}}
\newcommand{\mbW}{\mathbold{W}}
\newcommand{\mbX}{\mathbold{X}}
\newcommand{\mbY}{\mathbold{Y}}
\newcommand{\mbZ}{\mathbold{Z}}

\newcommand{\mbalpha}{\mathbold{\alpha}}
\newcommand{\mbbeta}{\mathbold{\beta}}
\newcommand{\mbdelta}{\mathbold{\delta}}
\newcommand{\mbepsilon}{\mathbold{\epsilon}}
\newcommand{\mbchi}{\mathbold{\chi}}
\newcommand{\mbeta}{\mathbold{\eta}}
\newcommand{\mbgamma}{\mathbold{\gamma}}
\newcommand{\mbiota}{\mathbold{\iota}}
\newcommand{\mbkappa}{\mathbold{\kappa}}
\newcommand{\mblambda}{\mathbold{\lambda}}
\newcommand{\mbmu}{\mathbold{\mu}}
\newcommand{\mbnu}{\mathbold{\nu}}
\newcommand{\mbomega}{\mathbold{\omega}}
\newcommand{\mbphi}{\mathbold{\phi}}
\newcommand{\mbpi}{\mathbold{\pi}}
\newcommand{\mbpsi}{\mathbold{\psi}}
\newcommand{\mbrho}{\mathbold{\rho}}
\newcommand{\mbsigma}{\mathbold{\sigma}}
\newcommand{\mbtau}{\mathbold{\tau}}
\newcommand{\mbtheta}{\mathbold{\theta}}
\newcommand{\mbupsilon}{\mathbold{\upsilon}}
\newcommand{\mbvarepsilon}{\mathbold{\varepsilon}}
\newcommand{\mbvarphi}{\mathbold{\varphi}}
\newcommand{\mbvartheta}{\mathbold{\vartheta}}
\newcommand{\mbvarrho}{\mathbold{\varrho}}
\newcommand{\mbxi}{\mathbold{\xi}}
\newcommand{\mbzeta}{\mathbold{\zeta}}

\newcommand{\mbDelta}{\mathbold{\Delta}}
\newcommand{\mbGamma}{\mathbold{\Gamma}}
\newcommand{\mbLambda}{\mathbold{\Lambda}}
\newcommand{\mbOmega}{\mathbold{\Omega}}
\newcommand{\mbPhi}{\mathbold{\Phi}}
\newcommand{\mbPi}{\mathbold{\Pi}}
\newcommand{\mbPsi}{\mathbold{\Psi}}
\newcommand{\mbSigma}{\mathbold{\Sigma}}
\newcommand{\mbTheta}{\mathbold{\Theta}}
\newcommand{\mbUpsilon}{\mathbold{\Upsilon}}
\newcommand{\mbXi}{\mathbold{\Xi}}

\newcommand{\mbzero}{\mathbold{0}}
\newcommand{\mbone}{\mathbold{1}}
\newcommand{\mbtwo}{\mathbold{2}}
\newcommand{\mbthree}{\mathbold{3}}
\newcommand{\mbfour}{\mathbold{4}}
\newcommand{\mbfive}{\mathbold{5}}
\newcommand{\mbsix}{\mathbold{6}}
\newcommand{\mbseven}{\mathbold{7}}
\newcommand{\mbeight}{\mathbold{8}}
\newcommand{\mbnine}{\mathbold{9}}


==> sec-background.tex <==
%!TEX root = main.tex
\section{BACKGROUND}\label{sec:background}
We present the background 
necessary for building 
the \acrlong{TopicRNN} model. We first review 
\acrshort{RNN}-based language modeling, followed by a discussion 
on the construction of latent topic models. 

% ======================================================================
%   LANGUAGE MODELING
% ======================================================================
\subsection{Recurrent Neural Network-Based Language Models}

Language modeling is %an important tool that is used for many
fundamental to many
applications. Examples include speech 
recognition and machine translation. 
%, such as speech recognition and machine translation. 
A language model is a probability distribution 
over a sequence of words
in a predefined vocabulary. More formally, let $V$ be a
vocabulary set and $y_1, ..., y_T$ a sequence 
of $T$ words with each $y_t\in V$.
A language model measures the likelihood of a 
sequence through a joint probability distribution,
\begin{equation*}
p(y_1, ..., y_T) = p(y_1)\prod_{t=2}^{T} p(y_t | y_{1: t-1}).
\end{equation*}
Traditional $n$-gram and feed-forward neural network language
models~\citep{bengio2003neural} typically make 
Markov assumptions about the sequential
dependencies between words, where the chain rule shown 
above limits conditioning to a fixed-size context window.

\acrshort{RNN}-based language models~\citep{mikolov2011extensions} 
sidestep this Markov assumption by defining the 
conditional probability of each word $y_t$ given all the 
previous words $y_{1:t-1}$ 
through a hidden state $h_t$ (typically via a softmax function):
%where $h_t$ is characterized by a \gls{RNN}, 
\begin{align*}
  p(y_t | y_{1: t-1}) &\triangleq p(y_t | h_t),  \\
  h_t & = f(h_{t-1}, x_t).
\end{align*}
The function $f(\cdot)$ can either be a 
standard \acrshort{RNN} cell or a more complex 
cell such as GRU~\citep{cho2014learning} 
or LSTM~\citep{hochreiter1997long}. The input and target words 
are related via the relation $x_t \equiv y_{t-1}$. 
%Such models 
These \acrshort{RNN}-based language models
have been quite successful~\citep{mikolov2011extensions,chelba2013one,jozefowicz2016exploring}.
%for language modeling~\citep{mikolov2011extensions,chelba2013one,jozefowicz2016exploring}.

While in principle \acrshort{RNN}-based models can ``remember''
arbitrarily long histories if provided enough capacity, in
practice such large-scale neural networks can easily encounter difficulties 
during optimization~\citep{bengio1994learning,pascanu2013difficulty,sutskever2013training} or
overfitting issues~\citep{srivastava2014dropout}. 
Finding better ways to model
long-range dependencies in language modeling is therefore 
an open research challenge. As motivated in the
introduction, much of the long-range dependency
in language comes from semantic coherence, %and 
not from syntactic structure 
%since syntax is 
which is
more of a local phenomenon. 
%Adji: Jianfeng does not like the sentence below...
%He suggested replacing it with the sentence below it
%Therefore, a method 
%that directly models long-range semantic dependencies 
%in language can make the task of capturing 
%local dynamics in language with an \gls{RNN} easier.
Therefore, models that can capture long-range
semantic dependencies in language are complementary
to \acrshort{RNN}s. In the following section, we describe 
a family of such models called probabilistic topic models.

%%N gram based\\
%%Feedforward neural nets\\
%%recurrent neural nets
%Language modeling is an important task that is used in speech recognition, machine translation, 
%information retrieval and many more applications. A language model is a probability distribution 
%over a sequence of words in a predefined set of eligible words -- also called a vocabulary. 
%More formally, denote by $V$ the vocabulary.  
%Denote by $x_1, ..., x_T$ a sequence of $T$ words in $V$. 
%A language model measures the likelihood of this sequence $p(x_1, ..., x_T)$.
%The chain rule of probability tells us that 
%\begin{equation*}
%p(x_1, ..., x_T) = p(x_1)\prod_{i=2}^{T} p(x_i | x_{1: i-1})
%\end{equation*}
%Computing these conditional probabilities is the language modeling task.
%There are many solutions to this language modeling task including $n$-gram models, 
%feed-forward neural network-based language models and recurrent neural network-based language models.\\
%The traditional $n$-gram models make Markov assumptions about the dependencies between the words
% in the sequence. The unigram model for example corresponds to the bag-of-word model and considers 
% all the words in the sequence as independent. The bigram model assumes the current word only depends 
% on the previous word. The $n$-gram model considers only the previous $n-1$ words in the sequence. 
% The corresponding joint distribution of the sequence $x_1,...,x_T$ in this case is
%\begin{equation*}
%p(x_1,...,x_T) = \prod_{i=1}^{T} p(x_i | x_{i-1 : i-n+1})
%\end{equation*}
%The problem with these $n$-gram models is that they do not have memory. In general when $n \geq 4$ the 
%conditional predictive probabilities above will be zero because of the curse of dimensionality. 
%Some line of work has proposed smoothing as a solution for this problem of vanishing probabilities. 
%However the memory problem is still present.\\
%Feed-forward neural network-based language models address this curse of dimensionality issue 
%by parameterizing the conditional probabilities with a feed-forward neural network. This type of language model takes the concatenation of the one-hot vector representation of the previous $n$ words as input. This vector is then passed to the hidden layers of the network which applies a nonlinear activation function such as sigmoid or hyperbolic tangent to this input. The predictive distribution of the next word is then computed by applying the softmax function to the output of the final hidden layer. This model is parameterized by the global weight matrices of the networks thus preventing the curse of dimensionality problem of $n$-gram models. These feed-forward neural network-based language models however still assume a fixed context window.\\
%Recent advances in language modeling replace the feed-forward neural network with a recurrent neural network. Theoretically, an RNN has the capacity of encoding dependencies between all the words preceding the current word. They do so via a recurrence relation in their hidden state. This however does not hold practically as vanishing and exploding gradients issues are incurred during training. Practically the gradient is estimated via truncated back propagation through time and clipping.\\
%Truncating the RNN takes away the capacity of the RNN to remember long range dependencies. Current solutions include using a different network architecture such as Gated-Recurrent Units and Long-Short Term Memory or providing context to the truncated RNN. Our work deals with the latter. This line of work consists in learning context features such as topics and providing this as context to the RNN either as a bias in the hidden layers or as a bias in the output layer or a combination of both.  

% ======================================================================
%    TOPIC MODELS
% ======================================================================
\subsection{Probabilistic Topic Models}
Probabilistic topic models are a family of models 
that can be used to capture global
semantic coherency \citep{blei2009topic}. 
They provide a powerful tool for
summarizing, organizing, and navigating document collections. 
One basic goal of such models is to find groups of words that tend to
co-occur together in the same document. 
These groups of words are called topics and
represent a probability distribution 
that puts most of its mass on this subset of the vocabulary. 
Documents are then represented as 
%a 
mixtures over these latent topics. 
Through posterior inference, the learned topics capture the 
semantic coherence of the words they cluster 
together~\citep{mimno2011optimizing}.

The simplest topic model is latent Dirichlet allocation
(LDA)~\citep{blei2003latent}.  It assumes $K$ underlying topics $\beta
= \{\beta_1,\dots,\beta_K\}$ , each of which is a distribution over a fixed
vocabulary. The generative process of LDA is as follows:\\
First generate the $K$ topics, $\beta_k \sim_{iid} {\rm Dirichlet}(\tau)$. 
Then for each document containing words $y_{1:T}$, 
independently generate document-level variables and data:
\begin{enumerate}
  \item Draw a document-specific topic proportion vector $\theta\sim {\rm Dirichlet}(\alpha)$. 
  \item For the $t$th word in the document,
\begin{enumerate}
  \item Draw topic assignment $z_t \sim {\rm Discrete}(\theta)$. 
  \item Draw word $y_t \sim {\rm Discrete}(\beta_{z_t})$. 
\end{enumerate}
\end{enumerate}
Marginalizing each $z_t$, we obtain the probability of
$y_{1:T}$ via a matrix factorization followed 
by an integration over the latent variable $\theta$,
\begin{align}
  p(y_{1:T} |\beta) = \int p(\theta)\prod_{t=1}^T \sum_{z_t} p(z_t |\theta)p(y_t | z_t,
\beta) {\rm d}\theta =\int p(\theta) \prod_{t=1}^T (\beta \theta)_{y_t} {\rm d}\theta.\label{eq:lda-prob}
\end{align}
In LDA the prior distribution on the topic proportions
is a Dirichlet distribution; it can be replaced by many 
other distributions. For example, the correlated topic 
model~\citep{blei2006correlated} uses a log-normal distribution.
Most topic models are ``bag of words'' models in that 
word order is ignored. This makes it easier for topic models to
capture global semantic information. However, this is also one of
the reasons why topic models %often do not make for good
%general-purpose language models. 
do not perform well on general-purpose
language modeling %tasks 
applications such as word prediction.
While bi-gram topic
models have been proposed~\citep{wallach2006topic}, 
higher order models quickly become intractable.

Another issue encountered by topic models is that they do not
model stop words well. This is because %: 1) stop words usually do not
 stop words usually do not carry semantic meaning; %-- 
 their appearance is mainly 
to make the sentence more readable according to the 
grammar of the language.
 They also appear frequently in almost every document 
 and can co-occur with almost
any word\footnote{\cite{wallach2009rethinking} described using
  asymmetric priors to alleviate this issue. Although it is not clear
how to use this idea in \acrlong{TopicRNN}, %the model we will present, 
 we plan to investigate such priors in future work.}.
 In practice, these stop words 
are chosen using tf-idf~\citep{blei2009topic}.%\\\\ 
 
 %In practice, these stop words 
%are chosen using tf-idf~\citep{blei2009topic}.

%Topic modeling is
%a sub-field of probabilistic modeling which consists in encoding the
%underlying hidden structure in data $\mbx$ in a set of latent
%variables $\mbz$ and positing a joint distribution $p(\mbx, \mbz)$ of
%the data and these latent variables. Discovering these hidden
%structures is done by learning the conditional distribution of the
%latent variables conditional on the data.  This distribution is called
%the posterior distribution and is denoted by $p(\mbz \g \mbx)$.

%Latent Dirichlet Allocation (LDA) is a classic example of topic model.
%It is applied to uncover the latent semantic structure of a corpus of
%documents.  This latent semantic structure is the set of topics --
%distributions over words -- pervading the document corpus.  In LDA
%each document is uniquely represented as vector. This vector
%represents the topic proportions of the document.  A document is thus
%a mixture of these topics. Each word in a given document is assumed to
%be assigned and generated from one of the topics. These modeling
%assumptions allow topic models such as LDA to capture global
%properties of documents i.e. which topics they exhibit. A shortcoming
%of these topic models is that they cannot address the task of
%predicting the next word in a sequence of words.  What they can do is
%provide the global properties of blocks of text.
%


% ======================================================================
%    NEURAL VARIATIONAL INFERENCE
% ======================================================================

%\iffalse
%\subsection{Neural Variational Inference}
%Language modeling is crucial to many natural language processing tasks. 
%Applications include machine translation, speech recognition and conversation systems. 
%In all these tasks, the performance of the language model is superior when long range 
%dependencies between words are correctly captured.  
% In this paper, we propose TopicRNN, a hybrid language and topic model that integrates 
% the merits of \gls{RNNs} with that of topic models. 
% More specifically, we let the RNN spend more of its capacity 
% to model local sequence structures and we provide it with long range semantic information 
% as usually captured by topic models. This contextual information is learned jointly 
% with the recurrent neural network parameters via an inference network. 
% Empirical results on the language modeling and sentiment analysis tasks 
% show superiority of our approach over other contextual recurrent neural network models. 
% We report competitive per-word perplexity on the Penn Treebank dataset and a new state of the art 
% error rate on the IMDB dataset.
% \fi
 


==> sec-discussion.tex <==
%!TEX root = main.tex

\section{DISCUSSION AND FUTURE WORK}\label{sec:discussion}
In this paper we introduced \acrlong{TopicRNN}, 
a \acrshort{RNN}-based language model that combines 
\acrshort{RNN}s and latent topics to capture
local (syntactic) and global (semantic) dependencies 
between words.
%hybrid language and topic 
%model that integrates the merits of recurrent neural networks with that 
%of topic models. \acrlong{TopicRNN} lets its recurrent neural network component 
%spend more of its capacity to model local sequence structures and its 
%document embedding
%encoder component provides the long range semantic information as context to the \acrshort{RNN}. 
The global dependencies as captured by the latent topics
serve as contextual bias to 
an \acrshort{RNN}-based language model.
This contextual information is learned jointly with the 
\acrshort{RNN} parameters by maximizing the evidence lower bound 
of variational inference. \acrlong{TopicRNN} yields competitive 
per-word perplexity on the Penn Treebank dataset 
compared to previous contextual \acrshort{RNN} models. We have 
reported a competitive classification error 
rate for sentiment analysis on the IMDB 100K dataset.  
 We have also illustrated the capacity of 
\acrlong{TopicRNN} to generate sensible topics and text. \\
In future work, we will study the performance of \acrlong{TopicRNN} when stop words 
are dynamically discovered during training. We will also extend \acrlong{TopicRNN} 
to other applications where capturing context is important such as in dialog modeling. 
If successful, this will allow us to have a model that performs 
well across different natural language processing applications. 
%\clearpage


==> sec-experiments.tex <==
%!TEX root = main.tex

\section{EXPERIMENTS}\label{sec:experiments}
We assess the performance of our proposed \acrlong{TopicRNN} model on  
word prediction and sentiment analysis\footnote{Our code will be made publicly available for reproducibility.}. 
For word prediction we use the Penn TreeBank 
dataset, a standard benchmark for assessing 
new language models~\citep{marcus1993building}. 
For sentiment analysis we use the IMDB 100k 
dataset~\citep{maas2011learning}, also a 
common benchmark dataset for this application\footnote{These datasets are publicly available 
at \url{http://www.fit.vutbr.cz/~imikolov/rnnlm/simple-examples.tgz} 
and \url{http://ai.stanford.edu/~amaas/data/sentiment/}.}.
We use \acrshort{RNN}, LSTM, and GRU cells
in our experiments leading to \acrlong{TopicRNN}, 
\acrlong{TopicLSTM}, and \acrlong{TopicGRU}.
\begin{table}[!hbpt]
\caption{\label{tab:topics} Five Topics from 
the \acrlong{TopicRNN} Model with 100 Neurons and 
50 Topics on the PTB Data. (The word \textit{s{\&}p} 
below shows as \textit{sp} in the data.)}
\begin{center}
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{c|c|c|c|c}
\toprule
Law & Company& Parties & Trading & Cars\\ \midrule
law  & spending & democratic & stock & gm \\
lawyers & sales & republicans & s{\&}p & auto \\
judge & advertising & gop & price & ford \\
rights & employees & republican & investor & jaguar \\
attorney & state & senate & standard & car \\
court & taxes & oakland & chairman & cars \\
general & fiscal & highway & investors & headquarters \\
common & appropriation & democrats & retirement & british \\
mr  & budget & bill & holders &executives \\
insurance & ad & district & merrill & model \\\bottomrule
\end{tabular}}
\end{center}
\end{table}
\begin{figure*}[!hbpt]
   \centering
    {\includegraphics[scale=0.22]{theta_gru.pdf}}
    {\includegraphics[scale=0.22]{theta_gru2.pdf}} 
    {\includegraphics[scale=0.22]{theta_gru3.pdf}}
    \caption{Inferred distributions using TopicGRU on three different documents.
    The content of these documents is added on the appendix.
    This shows that some of the topics are being picked up
    depending on the input document.}
    \label{fig:theta}
\end{figure*}
\begin{table}[!hbpt]
    \caption{\acrlong{TopicRNN} and its counterparts exhibit lower perplexity scores across 
    different network sizes than reported in ~\citet{mikolov2012context}. 
    \label{tab:pp}
    \Cref{tab:a} shows per-word perplexity scores for 10 neurons. 
    \Cref{tab:b} and \Cref{tab:c} correspond to per-word 
    perplexity scores for 100 and 300 neurons respectively.
    These results prove TopicRNN has more generalization capabilities:
    for example we only need a TopicGRU with 100 neurons 
    to achieve a better perplexity than stacking 2 LSTMs with 
    200 neurons each: 112.4 vs 115.9)}
     \centering
    \begin{subtable}{0.5\columnwidth}
        \caption{}\label{tab:a}
       \begin{tabular}{lcc}
\toprule
10 Neurons	&Valid	&Test \\\midrule
\acrshort{RNN} (no features) &$239.2$&$225.0$ \\
\acrshort{RNN} (LDA features)	 &$197.3$	 &$187.4$ \\
TopicRNN	 &$184.5$	 & $172.2$\\
TopicLSTM & $188.0$ & $175.0$\\
TopicGRU & $178.3$ & \bf{166.7} \\\bottomrule
\end{tabular}
    \end{subtable}
    \hspace{5pt}
    \begin{subtable}{0.4\columnwidth}
        \caption{}\label{tab:b}
        \begin{tabular}{lcc}
\toprule
100 Neurons & Valid & Test \\\midrule
\acrshort{RNN} (no features)  & $150.1$ & $142.1$ \\
\acrshort{RNN} (LDA features) & $132.3$ & $126.4$ \\
TopicRNN	 &$128.5$	 & $122.3$\\
TopicLSTM & $126.0$ & $118.1$\\
TopicGRU & $118.3$ & \bf{112.4} \\\bottomrule
\end{tabular}
    \end{subtable} 
     \centering
     \begin{subtable}{.5\columnwidth}
      \centering
        \caption{}\label{tab:c}
        \begin{tabular}{lcc}
\toprule
300 Neurons & Valid & Test \\\midrule
\acrshort{RNN} (no features)  & $ - $ & $124.7$ \\
\acrshort{RNN} (LDA features) & $ - $ & $113.7$ \\
TopicRNN	 &$118.3$	 &$112.2$\\
TopicLSTM & $104.1$ & $99.5$\\
TopicGRU & $99.6$ & \bf{97.3} \\\bottomrule
\end{tabular}
    \end{subtable} 
\end{table}
\iffalse
\begin{table}[!hbpt]
\caption{Test perplexity reported on Penn TreeBank dataset. 
\acrlong{TopicGRU} provides the state of the art perplexity on this dataset.} 
\label{tab:test_perp}
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{lr}
\toprule
Model & Reported Test Perplexity\\\midrule
RNN-LDA + KN-5 + cache (Mikolov \& Zweig 2012) & $92.0$\\
Deep RNN (Pascanu et al. 2013) & $107.5$\\
Sum-Prod Net (Cheng et al., 2014) & $100.0$\\
LSTM large (Zaremba et al., 2014) & $78.4$ \\
Variational LSTM large (Gal 2015) & $73.4$ \\
CharCNN  (Kim et al., 2016) & $78.9$ \\
Variational RHN (Zilly et al., 2016) & $71.3$ \\
Pointer Sentinel LSTM (Merity et al. 2016) & $70.9$ \\
\midrule
TopicRNN & $0$\\
TopicLSTM & $0$\\
TopicGRU & \bf{0}\\\bottomrule
\end{tabular}}
\end{table}
\fi
\subsection{Word Prediction}
We first tested \acrlong{TopicRNN} on the word prediction 
task using the Penn Treebank (PTB) 
portion of the Wall Street Journal. We use the 
standard split, where sections 0-20 (930K tokens) 
are used for training, sections 21-22 (74K tokens) for 
validation, and 
sections 23-24 (82K tokens) for 
testing~\citep{mikolov2010recurrent}. 
We use a vocabulary of size $10K$ that includes 
the special token \textit{unk} for 
rare words and \textit{eos} that indicates the 
end of a sentence. \acrlong{TopicRNN} takes documents 
as inputs. We split the PTB data into blocks 
of 10 sentences to constitute documents 
as done by~\citep{mikolov2012context}. 
The inference network takes as input the bag-of-words 
representation of the input document. 
For that reason, the vocabulary size of the inference network is reduced 
to $9551$ after excluding $449$ pre-defined stop words. 

In order to compare with previous work on 
contextual \acrshort{RNN}s we trained \acrlong{TopicRNN}
 using different network sizes. We performed 
 word prediction using a recurrent neural 
 network with 10 neurons, 100 neurons and 300 
 neurons. For these experiments, we used 
 a multilayer perceptron with 2 hidden layers 
 and 200 hidden units per layer for the inference network. 
 The number of topics was tuned depending on 
 the size of the \acrshort{RNN}. For 10 neurons 
 we used 18 topics. For 100 and 300 neurons we found 50 
 topics to be optimal. We used the validation set 
 to tune the hyperparameters of the model.
 We used a maximum of 15 epochs for the experiments 
 and performed early stopping 
 using the validation set. For comparison purposes 
 we did not apply dropout and used 1 layer 
 for the \acrshort{RNN} and its counterparts in all 
 the word prediction experiments as reported in \Cref{tab:pp}.
One epoch for 10 neurons takes $2.5$ minutes.
For 100 neurons, one epoch is completed in less than 
4 minutes. Finally, for 300 neurons one epoch takes 
less than 6 minutes. These experiments were ran
on Microsoft Azure NC12 that has 12 cores, 2 Tesla K80 GPUs,
and 112 GB memory.
%We observed that the topics were more interpretable for smaller networks. 
\iffalse
\begin{figure*}[!hbpt]
   \centering
    {\includegraphics[scale=0.22]{theta_gru.pdf}}
    {\includegraphics[scale=0.22]{theta_gru2.pdf}} 
    {\includegraphics[scale=0.22]{theta_gru3.pdf}}
    \caption{Inferred distributions using TopicGRU on three different documents.
    The content of these documents is added on the appendix.
    This shows that some of the topics are being picked up
    depending on the input document.}
    \label{fig:theta}
\end{figure*}
\fi
First, we show five randomly drawn topics in \Cref{tab:topics}. These
results correspond to a network with 100 neurons.  We also illustrate
some inferred topic distributions for several documents from TopicGRU
in \Cref{fig:theta}. Similar to standard topic models, these
distributions are also relatively peaky.
%We also illustrate some inferred distributions from 
%TopicRNN, TopicLSTM, and TopicGRU in \Cref{fig:theta}.
%As can be seen they infer approximately the same distributions. 
 
Next, we compare the performance of \acrlong{TopicRNN}
to our baseline contextual \acrshort{RNN}
using perplexity. %as a performance measure for this task. 
 Perplexity can be thought of 
as a measure of surprise for a language model. It is 
defined as the exponential of the 
average negative log likelihood. \Cref{tab:pp} summarizes 
the results for different network sizes. 
We learn three things from these tables. First, 
the perplexity is reduced the larger 
the network size. Second, \acrshort{RNN}s with context 
features perform better 
than \acrshort{RNN}s without context features. Third, we 
see that \acrlong{TopicRNN} 
gives lower perplexity than the previous baseline result 
reported by~\cite{mikolov2012context}. Note that
to compute these perplexity scores for word prediction
we use a sliding window to compute $\theta$ as we move
along the sequences. The topic vector $\theta$ that is used 
from the current batch of words is estimated from 
the previous batch of words. This enables fair comparison 
to previously reported results \citep{mikolov2012context}.\footnote{We
adjusted the scores in \Cref{tab:pp} from what was previously reported
after correcting a bug in the computation of the ELBO.}

Another aspect of the \acrlong{TopicRNN} 
model we studied is its capacity to generate coherent text. 
To do this, we randomly drew a document from the test set
and used this document as seed input to the inference network 
to compute $\theta$. Our expectation is that 
the topics contained in this seed document 
are reflected in the generated text.
\Cref{tab:text} shows generated text from models 
learned on the PTB and IMDB datasets. See \Cref{sec:appendix_text} 
for more examples. 
\begin{table}[t]
\caption{\label{tab:text}Generated text using the \acrlong{TopicRNN} model 
on the PTB (top) and IMDB (bottom).}
\begin{center}
\begin{tabular}{l}
\begin{minipage}[t]{0.9\columnwidth}%
\textit{they believe that they had senior damages 
to guarantee and frustration of unk 
stations eos the rush to minimum effect in composite 
trading the compound base inflated rate 
before the common charter 's report eos wells 
fargo inc. unk of state control funds without openly 
scheduling the university 's exchange rate has been 
downgraded it 's unk said eos the united 
cancer \& began critical increasing rate of 
N N at N N to N N are less for the country 
to trade rate for more than three months \$ N workers were mixed eos}\vspace{3pt}
\end{minipage}\tabularnewline
\midrule\vspace{3pt}
\begin{minipage}[t]{0.9\columnwidth}%
\textit{lee is head to be watched unk month she 
eos but the acting surprisingly 
nothing is very good eos i cant believe that he 
can unk to a role eos may appear of 
for the stupid killer really to help with unk unk unk 
if you wan na go to it fell to the plot 
clearly eos it gets clear of this movie $70$ are 
so bad mexico direction regarding 
those films eos then go as unk 's walk and after unk 
to see him try to unk before that unk with this film}
\end{minipage}\tabularnewline
\end{tabular}
\end{center}
\end{table}

\subsection{Sentiment Analysis}
%classification error rates...
\begin{table}[t]
\caption{Classification error rate on IMDB 100k dataset. 
\acrlong{TopicRNN} provides the state of the art error rate on this dataset.} 
\label{tab:imdb}
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{lr}
\toprule
Model & Reported Error rate\\\midrule
BoW (bnc) (Maas et al., 2011) & $12.20\%$\\
BoW ($b\Delta$ t\'c) (Maas et al., 2011) & $11.77\%$\\
LDA (Maas et al., 2011) & $32.58\%$\\
Full +  BoW (Maas et al., 2011) & $11.67\%$ \\
Full + Unlabelled + BoW (Maas et al., 2011) & $11.11\%$ \\
WRRBM  (Dahl et al., 2012) & $12.58\%$ \\
WRRBM + BoW (bnc) (Dahl et al., 2012) & $10.77\%$ \\
MNB-uni (Wang \& Manning, 2012) & $16.45\%$ \\
MNB-bi (Wang \& Manning, 2012) & $13.41\%$ \\
SVM-uni (Wang \& Manning, 2012) & $13.05\%$ \\
SVM-bi (Wang \& Manning, 2012) & $10.84\%$ \\
NBSVM-uni (Wang \& Manning, 2012) & $11.71\%$ \\
seq2-bown-CNN (Johnson \& Zhang, 2014) & $14.70\%$ \\
NBSVM-bi (Wang \& Manning, 2012) & $8.78\%$ \\
Paragraph Vector (Le \& Mikolov, 2014) & $7.42\%$ \\
%\midrule
SA-LSTM  with joint training (Dai \& Le, 2015) & $14.70\%$ \\
LSTM with tuning and dropout (Dai \& Le, 2015)  & $13.50\%$ \\
LSTM initialized with word2vec embeddings (Dai \& Le, 2015) & $10.00\%$ \\
SA-LSTM  with linear gain (Dai \& Le, 2015) & $9.17\%$ \\
LM-TM  (Dai \& Le, 2015) & $7.64\%$ \\
SA-LSTM (Dai \& Le, 2015)  & $7.24\%$ \\
\textbf{Virtual Adversarial (Miyato et al. 2016)} & \textbf{5.91\%}\\
\midrule
\textbf{TopicRNN } & \textbf{6.28\%} \\\bottomrule
\end{tabular}}
\end{table}
%clustered documents from imdb
\begin{figure}[t]
\centering
\includegraphics[width=.95\textwidth]{clustersmoredocs.eps}
\caption{Clusters of a sample of $10000$ movie reviews from the IMDB $100$K 
dataset using \acrlong{TopicRNN} as feature extractor. We used K-Means to cluster
 the feature vectors. We then used PCA to reduce 
 the dimension to two for visualization purposes.
 \red{red} is a negative review and \green{green} is a positive review.}
\label{fig:clusters}
\end{figure}
We performed sentiment analysis using \acrlong{TopicRNN} 
as a feature extractor on 
the IMDB 100K dataset. This data consists 
of 100,000 movie reviews from 
the Internet Movie Database (IMDB) website. The 
data is split into $75\%$ for training and $25\%$ for testing. 
Among the 75K training reviews, 50K are unlabelled 
and 25K are labelled as carrying either a positive or a negative sentiment. 
All 25K test reviews are labelled. We trained 
\acrlong{TopicRNN} on 65K random training reviews and used 
the remaining 10K reviews for validation. To learn a classifier, we passed 
the 25K labelled training reviews through the learned \acrlong{TopicRNN} model. We 
then concatenated the output of the inference network and the last 
state of the \acrshort{RNN} for each of these 25K reviews to compute the feature vectors. 
We then used these feature vectors to train a neural network with one hidden 
layer, 50 hidden units, and a sigmoid activation function to predict sentiment, exactly as 
 done in~\citet{le2014distributed}. 
 
To train the \acrlong{TopicRNN} model, we used a vocabulary 
of size 5,000 and mapped all other words to the \textit{unk} token. 
We took out 439 stop 
words to create the input of the inference network. 
We used 500 units and 2 layers 
for the inference network, and used 2 layers 
and 300 units per-layer for the \acrshort{RNN}. 
We chose a step size of 5 and defined 200 topics. 
We did not use any regularization such as dropout. 
We trained the model for 13 epochs and used the 
validation set to tune the 
hyperparameters of the model and track perplexity 
for early stopping. This experiment took close to 78 hours
on a MacBook pro quad-core with 16GHz of RAM. 
See \Cref{sec:appendix_imdb_topics} for the 
visualization of some of the topics learned from this data.

\Cref{tab:imdb} summarizes sentiment classification results from
\acrlong{TopicRNN} and other methods.  Our error rate is
$6.28\%$.\footnote{The experiments were solely based on TopicRNN.
Experiments using TopicGRU/TopicLSTM are being carried out and will be
added as an extended version of this paper.}  This is close to the
state-of-the-art $5.91\%$~\citep{miyato2016adversarial} despite that
we do not use the labels and adversarial training in the feature
extraction stage.  Our approach is most similar
to~\citet{le2014distributed}, where the features were extracted in a
unsupervised way and then a one-layer neural net was trained for
classification.

%a relative $13.3\%$ improvement over 
% the previously reported 
%error rate by~\citep{dai2015semi}\footnote{this result is based on semi-supervised learning 
%whereas the result from TopicRNN is based on unsupervised learning:
%we first perform feature extraction and then train a one-layer 
%neural net classifier.}. 
%The error rates on other methods 
%are reported in~\citet{le2014distributed,dai2015semi,miyato2016adversarial}.

\Cref{fig:clusters} shows the ability of \acrlong{TopicRNN} to cluster documents 
using the feature vectors as created 
during the sentiment analysis task. 
Reviews with positive sentiment are coloured 
in green while reviews carrying 
negative sentiment are shown in red. This shows that 
\acrlong{TopicRNN} can be used as an unsupervised feature 
extractor for downstream applications.
\Cref{tab:text} shows generated text from models 
learned on the PTB and IMDB datasets. See \Cref{sec:appendix_text}
for more examples. The overall generated text from IMDB encodes a negative 
sentiment.


==> sec-introduction.tex <==
%!TEX root = main.tex

\section{INTRODUCTION}\label{sec:introduction}
%1. talk about language modeling, n-grams, feed-froward neural nets, rnnlm, contextual rnnlm
%2. discuss different papers working on the same thing
%3. discuss our approach at high level: solving vanishing gradient problem, leveraging new advances in neural vi, advantage of our approach (simplicity of the architecture, scalability, generalizability), discuss the similarity with neural vi for text paper and how we extend that work, discuss our handling of stop words
%4. highlight our contributions
%5. provide organization of the paper
%Recurrent neural network based  language models fail to fully capture these long range dependencies due to their well known problem of vanishing and exploding gradients. These long range dependencies largely depend on the semantic information in the text rather than the structural ordering of the words.
%\citep{mikolov2012context, ghosh2016contextual}
When reading a document, short or long, humans have a mechanism that
somehow allows them to remember the gist of what they have read so
far. Consider the following example:

``\textit{The \textcolor{blue}{U.S.}\textcolor{blue}{presidential}
  \textcolor{blue}{race} isn't only drawing attention and controversy
  in the \textcolor{blue}{United States} -- it's being closely watched
  across the globe. But what does the rest of the world think about a
  \textcolor{blue}{campaign} that has already thrown up one surprise
  after another?  CNN asked 10 journalists for their take on the
  \textcolor{blue}{race} so far, and what their  \textcolor{blue}{country} might be
hoping for in \textcolor{blue}{America}'s next
\textcolor{blue}{\bf{---}}}''

%Any human will quickly guess that the missing word in the text above
The missing word in the text above
is easily predicted by any human to be 
either \textit{President} or \textit{Commander in Chief} or their
synonyms. There have been various language models -- from simple $n$-grams
to the most recent \acrshort{RNN}-based language
models -- that aim to solve this problem of predicting correctly the
subsequent word in an observed sequence of words. 

A good language model should capture at least two important properties
of natural language. %the language. 
 The first one is correct syntax. 
In order to do prediction that enjoys this property, 
we often only need to consider a few preceding words. 
Therefore, correct syntax is more of a local property.
Word order matters in this case. 
The second property is the semantic coherence of the prediction. To achieve
this, we often need to consider many preceding words to understand the %long-range
global %semantic dependency 
semantic meaning of the sentence or document. 
%However, when we consider this semantic dependency, 
%the actual syntax structure 
The ordering of the words usually matters much less in this case.

%Adji: pepper the rest of the introduction with references
Because they only consider a fixed-size context
window of preceding words,
traditional $n$-gram and neural probabilistic language
models~\citep{bengio2003neural} have difficulties in capturing
%long-range dependency 
global semantic information. %since they only consider a fixed-size context window of preceding words. 
To overcome this, \acrshort{RNN}-based 
language models~\citep{mikolov2010recurrent,mikolov2011extensions} 
use hidden states to
``remember'' the history of a word sequence. However, 
%in none of these
%models is there an explicit modeling of the two language properties
none of these approaches explicitly model the two main 
properties of language %properties
mentioned above, correct syntax and semantic coherence. 
Previous work by \cite{chelba2000structured} and \cite{gao2004dependence}
%considered approaches that do not 
%involve neural networks to capture long-range dependencies in 
%language~\citep{chelba2000structured, gao2004dependence}.
exploit syntactic or semantic parsers to capture
long-range dependencies in language.
%Adji: i commented out the sentence below because it is unclear.
%However, mixing
%them together might not be the best strategy, since syntax
%tends to be a local property and semantic a global one. 

In this paper, we propose \acrlong{TopicRNN}, a \acrshort{RNN}-based
language model that is designed to directly capture long-range
semantic %dependency 
dependencies via latent topics. These topics provide context
to the \acrshort{RNN}.
 Contextual \acrshort{RNN}s have received 
a lot of attention~\citep{mikolov2012context, mikolov2014learning, ji2015document, lin2015hierarchical, ji2016latent, ghosh2016contextual}.
 However, the models
closest to ours are the contextual \acrshort{RNN} model proposed
by~\cite{mikolov2012context} %along with 
and its most recent extension to
the long-short term memory (LSTM)
architecture~\citep{ghosh2016contextual}. %-- which 
These models use pre-trained
topic model features as an additional input to the hidden states
and/or the output of the \acrshort{RNN}. In contrast, \acrlong{TopicRNN} does
not require pre-trained topic model features and can be learned in an
end-to-end fashion. %, and 
%We also have a different modeling motivation. 
We introduce an automatic way for handling
stop words that topic models usually have difficulty dealing with.
Under a comparable model size set up, \acrlong{TopicRNN} achieves better
perplexity scores than the contextual \acrshort{RNN}
model of~\citet{mikolov2012context} on the Penn TreeBank dataset
\footnote{\citet{ghosh2016contextual} did not 
publish results on the PTB and we did not find the code online.}.
Moreover, \acrlong{TopicRNN} can be used as an unsupervised feature extractor
for downstream applications. For example, we derive document features
of the IMDB movie review dataset using \acrlong{TopicRNN} for
sentiment classification. We reported an error rate of $6.28\%$. This
is close to the state-of-the-art
$5.91\%$~\citep{miyato2016adversarial} despite that we do not use the
labels and adversarial training in the feature extraction stage.

%We achieve %a state-of-the-art error rate, 
%a $13.3\%$ improvement
%over the previously %best result
%reported state-of-the-art error rate~\citep{dai2015semi}. 

The remainder of the paper is organized as follows: 
\Cref{sec:background} provides background on \acrshort{RNN}-based language models and
probabilistic topic models. \Cref{sec:TOPICRNN} 
describes the \acrlong{TopicRNN} network architecture,
its generative process and how to perform inference for it. 
\Cref{sec:experiments} presents per-word perplexity 
results on the Penn TreeBank dataset
and the classification error rate on the IMDB $100$K dataset.  
Finally, %in \Cref{sec:relatedwork} we highlight some related work before 
we conclude and provide future research directions in \Cref{sec:discussion}. 
%
%This problem is solved by feed-forward neural network
%language models such as the neural probabilistic language model of
%. However these networks, just like $n$-grams,
%consider a fixed context window and cannot capture global semantic
%information such as topics. Recent advances in language modeling
%replace the feed-forward network with an RNN which theoretically,
%because of its internal recurrent connections, has the capacity to
%remember all the text preceding the current word.  However, RNNs do
%not practically have the capacity to remember all the preceding words
%due to their vanishing/exploding gradients
%issue~\citep{bengio1994learning, pascanu2013difficulty}.
%

% chong: moved to into main text/related work.
%The solution to this problem is to truncate the RNN to look back up to
%a certain point in time and boost its performance with contextual
%information.  \citep{mikolov2012context} pioneered this work around
%providing context to RNNs.  They do so by first training a topic model
%such as LDA \citep{blei2003latent} and using the topic output as
%context features to an RNN-based language model.

%
%We propose many improvements to this approach leading to the TopicRNN
%model architecture.  Our contributions are as follows:
%
%\begin{itemize}[leftmargin=*]
%
%\item We solve the vanishing/exploding gradients problem of RNNs by choosing 
%a low number of steps and providing context. This has the advantage of making the best 
%out of the RNN while providing it with the required memory to better predict the upcoming word.
%
%\item We learn the contextual information jointly with the network parameters: 
%this has the advantage of boosting the performance of the language model 
%since the right information needed is captured and not extraneous.
%
%\item We model stop words via binary classification: 
%topic models do not handle stop words, they get rid of them. 
%Language models need to predict stop words as well as content words. 
%We reconcile the language model and the topic model when it comes to these stop words 
%by modeling them and thus providing the RNN with contextual information 
%only when the target word is a content word. 
%
%\item We report state of the art results on the language modeling and sentiment analysis task.
%
%\end{itemize}
%
%\iffalse
%In this paper, we present a new way of bringing contextual information to 
%recurrent neural network based language models. In this new approach 
%we solve the vanishing/exploding gradients problem of recurrent neural networks 
%and learn the contextual information along with the network parameters thus avoiding 
%the two stage process of running another model to get the contextual information. 
%Discuss approaches similar to ours. In contrast to these approaches we choose 
%a vanilla RNN architecture and jointly learn the contextual information along with 
%the model parameters via an inference network. We also model stop words 
%via binary classification which has not been done before in these language models.\\
%The contributions of this paper are as follows:\\\\
%\fi
%
%The remainder of the paper is organized as follows: 
%Section 2 provides some background on language modeling, 
%neural variational inference and topic models. 
%Section 3 describes the TopicRNN network architecture, 
%its generative process and its scalable version. 
%Section 4 presents per-word perplexity results on the Penn TreeBank datasets 
%and classification error rate on the IMDB 100k dataset. 
%Finally, in Section 5 we highlight some related work before 
%concluding and providing future directions in Section 6. 




==> sec-relatedwork.tex <==
%!TEX root = main.tex
\section{RELATED WORK}\label{sec:relatedwork}
\parhead{Vector representations of documents:} 
Learning vector representations of documents is an important machine learning task. 
Topic modeling~\citep{blei2012probabilistic, blei2009topic} represents each document 
as a vector of topic proportions by discovering the latent semantic structure of a corpus 
of documents. Many topic models -- parametric and nonparametric -- have 
been successfully applied for this: \citep{blei2003latent, blei2010nested, 
mimno2012topic, griffiths2004finding, teh2012hierarchical, blei2006correlated}. 
Other approaches to document modeling use neural networks~\citep{larochelle2012neural, 
srivastava2013modeling, miao2015neural, le2014distributed}. Our representation of 
documents is closest to the work by~\citep{miao2015neural} who 
use a VAE~\citep{kingma2013auto} approach to document modeling.
 This consists in using a feed-forward neural network that takes a bag-of-word 
 representation of a document and learns a lower dimensional vector representation 
 of the document by jointly training the encoder and the generative model of the document. 
 Our work differs from theirs in how we generate back the document and how 
 we use the output of the inference network.
 
\parhead{Language modeling:} 
Feed-forward neural network-based language models address the 
curse of dimensionality issue of n-gram models~\citep{bengio2003neural, schwenk2007continuous, 
mnih2007three, le2011structured, hai2012measuring}. However, they still consider a fixed context window. 
This issue is alleviated by RNN-based language models~\citep{mikolov2011extensions, mikolov2010recurrent} 
that use recurrent connections in their hidden layers. Training RNNs with long recurrence can be difficult~\citep{bengio1994learning, pascanu2013difficulty, sutskever2013training}. 
There has been a lot of work dedicated to solving this issue. One approach is to use
a small context window and/or add additional context 
features~\citep{mikolov2012context, ghosh2016contextual, ji2015document, lin2015hierarchical, ji2016latent}. 
Another approach is to use a different architecture such as LSTM and GRU~\citep{hochreiter1997long, cho2014learning}. 
Our work lies within the first category. %Unlike~\citep{} we jointly learn the context features along with the model parameters. 
The closest related work is~\citep{mikolov2014learning}. Our work complements theirs in two ways. 
We model stop words and provide the context feature as bias to only the output layer of the 
RNN generative model contrary to their approach of feeding this context feature both to the 
hidden layer and output layer of the RNN. This results in a end-to-end learned model and lower perplexity scores.

%In this paper, we propose a model that learns a distributed representation 
%of documents and provide these learned vectors as bias to an RNN-based language model.

==> sec-topicrnn.tex <==
%!TEX root = main.tex

\section{The \acrlong{TopicRNN} Model}\label{sec:TOPICRNN}
\begin{figure*}[t]
  \begin{subfigure}{.47\textwidth}
\centering
\includegraphics[width=0.95\textwidth]{unrolled.pdf}
\caption{}
\end{subfigure}
\begin{subfigure}{.56\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{model.pdf}
\caption{}
  \end{subfigure}
  \caption{(a) The unrolled \acrlong{TopicRNN} architecture: $x_1, ..., x_6$
  	are words in the document, $h_t$ is the state of the \acrshort{RNN} at time step $t$, 
	$x_i \equiv y_{i-1}$, $l_1, ..., l_6$ are stop word indicators, and
	$\theta$ is the latent representation of the input document
    and is unshaded by convention. (b) The
     \acrlong{TopicRNN} model architecture in its compact form: 
     	$l$ is a binary vector that indicates whether each word in 
	the input document is a stop word or not. Here \red{red} indicates stop words
	and \blue{blue} indicates content words.}
\label{fig:architecture}
\end{figure*}

We next describe the proposed \acrlong{TopicRNN}
model. In \acrlong{TopicRNN}, latent topic models are used to capture
global semantic dependencies so that the \acrshort{RNN} can focus its modeling capacity
on the local dynamics of the sequences. With this joint
modeling, we hope to achieve better overall performance on downstream
applications.

\parhead{The model.} \acrlong{TopicRNN} is a generative model. For a document containing the words $y_{1:T}$, 
\begin{enumerate}
  \item Draw a topic vector\footnote{Instead of using the Dirichlet distribution,
    we choose the Gaussian distribution. This allows for more flexibility in
  the sequence prediction problem and also has advantages during inference.}
    $\theta\sim N(0,I)$. 
  \item Given word $y_{1:t-1}$, for the $t$th word $y_t$ in the document,
\begin{enumerate}
  \item Compute hidden state $h_t = f_W(x_t, h_{t-1})$, where we let $x_t \triangleq y_{t-1}$.  
  \item Draw stop word indicator $l_t \sim {\rm Bernoulli}(\sigma(\Gamma^\top h_t))$, with $\sigma$ the sigmoid function.
  \item Draw word $y_t \sim p(y_t | h_t, \theta, l_t,B)$, where
  \begin{align*}
  p(y_t = i | h_t, \theta, l_t,B) \propto \exp\left(v_i^\top h_t  + (1-l_t) b_i^\top\theta\right).
\end{align*}
\end{enumerate}
\end{enumerate}

The stop word indicator $l_t$ controls how the topic vector $\theta$ affects the output. 
If $l_t = 1$ (indicating $y_t$ is a stop word), the topic vector
$\theta$ has no contribution to the output. Otherwise, we add a bias
to favor those words that are more likely to appear when 
mixing with $\theta$, as measured by the dot product 
between $\theta$ and the latent word vector $b_i$ for the $i$th vocabulary word.  
As we can see, the long-range semantic
information captured by $\theta$ directly
affects the output through an additive procedure. Unlike~\citet{mikolov2012context}, the contextual
information is not passed to the hidden layer of the \acrshort{RNN}.
The main reason behind our choice of using the topic vector as bias
instead of passing it into the hidden states of the RNN is because
it enables us to have a clear separation of the contributions of global
semantics and those of local dynamics. The global semantics come from
the topics which are meaningful when stop words are excluded. 
However these stop words are needed for the local dynamics of the language
model. We hence achieve this separation of global vs local via a
binary decision model for the stop words.
It is unclear how to achieve this if we pass the topics to the hidden
states of the RNN. This is because the hidden states of the RNN will
account for all words (including stop words) whereas the topics
exclude stop words.  
%Passing the topics through the hidden states of
%the RNN violates this.  

We show the unrolled graphical representation of \acrlong{TopicRNN} in
\Cref{fig:architecture}(a). 
We denote all model parameters 
as $\Theta = \{\Gamma, V, B, W, W_c\}$ (see \Cref{sec:appendix_params}
for more details). Parameter $W_c$ is for the inference network, which
we will introduce below.
%Adji: reformulate the sentence below or put it after ELBO
%The model parameters $\Gamma$, $V = \{v_{1:V}\}$,
%$\boldsymbol{b} = \{b_{1:V}\}$, $W$---the RNN 
%cell parameters in $f_W(\cdot)$---are to be learned.  
The observations are the word sequences $y_{1:T}$ and stop word
indicators $l_{1:T}$.\footnote{Stop words can be determined using one of 
the several lists available online. For example, 
\url{http://www.lextek.com/manuals/onix/stopwords2.html}}
The log marginal likelihood of the sequence
$y_{1:T}$ is
\begin{align}
  \log p(y_{1:T}, l_{1:T}|h_t) = \log \int p(\theta) \prod_{t=1}^T p(y_t | h_t, l_t, \theta) p(l_t
  | h_t) {\rm d} \theta. \label{eq:likelihood}
\end{align}

\parhead{Model inference.} Direct optimization of
\Cref{eq:likelihood} is intractable so we use variational
inference for approximating this 
marginal~\citep{jordan1999introduction}. Let $q(\theta)$ be the
variational distribution on the marginalized variable $\theta$. 
We construct the variational objective function, also called 
the evidence lower bound (\acrshort{ELBO}), as follows:
\begin{align*}
  \mathcal{L}(y_{1:T}, l_{1:T}|q(\theta), \Theta) &\triangleq~
  \EE{q(\theta)} {\sum_{t=1}^T  \log p(y_t | h_t, l_t, \theta) + \log p(l_t
  | h_t) + \log p(\theta) - \log q(\theta)} \\ 
  & \leq ~\log p(y_{1:T}, l_{1:T} |h_t,\Theta).
\end{align*}
Following the proposed variational autoencoder 
technique, we choose the form of
$q(\theta)$ to be an inference network using a feed-forward neural
network~\citep{kingma2013auto,miao2015neural}. 
Let $X_c\in \mathcal{N}_+^{|V_c|}$
be the term-frequency representation of $y_{1:T}$ {\it excluding} 
stop words (with $V_c$ the vocabulary size without the
stop words). The variational autoencoder inference 
network $q(\theta|X_c, W_c)$ with parameter
$W_c$ is a feed-forward neural network with ReLU activation units that
projects $X_c$ into a $K$-dimensional latent space. Specifically,  we
have
\begin{align*}
	q(\theta | X_c, W_c) &= N(\theta; \mu(X_c), \diag(\sigma^2(X_c))), \\
  \mu(X_c) &= W_1 g(X_c) + a_1,\\
	\log\sigma(X_c) &= W_2 g(X_c) + a_2,
\end{align*}
where $g(\cdot)$ denotes the feed-forward neural network. The weight
matrices $W_1$, $W_2$ and biases $a_1$, $a_2$ are shared across
documents. Each document has its own $\mu(X_c)$ and $\sigma(X_c)$
resulting in a unique distribution $q(\theta | X_c)$ for each
document.  The output of the inference network is a
distribution on $\theta$, which we regard as the
summarization of the semantic information, similar to the topic
proportions in latent topic models. We show the role of the inference
network in \Cref{fig:architecture}(b).  During training, the
parameters of the inference network and the model are jointly learned
and updated via truncated backpropagation through time using the
Adam algorithm~\citep{kingma2014adam}. We use stochastic samples from
$q(\theta|X_c)$ and the reparameterization
trick towards this end~\citep{kingma2013auto,rezende2014stochastic}.


%In this section we describe how to marry latent topic modeling with 
%recurrent neural network-based language modeling. 
%\citep{mikolov2012context} pioneered the idea of incorporating topic 
%features as context to an RNNLM. They do so by separately training an LDA 
%model and using the topic matrix as input to the hidden and output layers of an RNNLM. 
%This resulted in significantly better perplexity scores and higher accuracy
%in speech recognition. In this paper, we learn the context features jointly with 
%the parameters of the RNN using ideas from variational autoencoders and 
%neural variational inference. We go another step further and distinguishing 
%between generating a stop word or a content word via binary classification. 
%TopicRNN combines a stochastic distributed representation of a document with a RNN 
%generative model to achieve state of the art classification error rate on the IMDB dataset.\\\\
% =====================================================================
%   MODEL AND ARCHITECTURE
% ======================================================================
%\parhead{Model and Architecture:}
%TopicRNN in \Cref{fig:architecture} is a generative model of text that extracts a stochastic 
%continuous representation of a document. This distributed representation encodes semantic 
%information that is used as additional bias to a \gls{RNN} generative model.
%TopicRNN extends a classic VAE in three ways:
%\begin{itemize}[leftmargin=*]
%	\item the decoder is a RNN instead of a simple MLP
%	\item the decoder has an extra stop word predictor 
%		that decides whether to predict a stop word 
%		or a content word by conditioning on the hidden layer of the RNN
%	\item the output of the encoder is provided as bias directly to the output of the decoder
%		and not passed to the hidden layer of the decoder.
%\end{itemize}
%At a high level TopicRNN works as follows:
%an MLP encoder takes a bag-of-words representation of a document as input and compresses it
%into a continuous latent distribution. A softmax decoder predicts each word in the document 
%by condition on the hidden layer of a jointly trained RNN, a stop word predictor, and 
%the vector representation of the document.\\\\
%% ======================================================================
%% ENCODER
%% ======================================================================
%\parhead{Encoder:}
%Let $D$ be an input document. Let $X\in R^{|V|}$ be its bag-of-words representation 
%that excludes stop words. 
%The encoder of the model is a feed-forward neural network with ReLU activation units 
%that projects $X$ into a $K$-dimensional latent space. 
%The resulting K-dimensional vector representation of $X$
%denoted by $\theta$ is obtained by sampling from the variational distribution $q(\theta | X)$ 
%whose parameters are outputs of the feed-forward neural network. We choose:
%\begin{align*}
%	q(\theta | X) &= N(\theta; \mu(X), \diag(\sigma^2(X))) \\
%	\mu(X) &= W_1 f(X) + b_1\\
%	\log\sigma(X) &= W_2 f(X) + b_2
%\end{align*}
%where $f$ denotes the feed-forward neural network. The weight matrices 
%$W_1$, $W_2$ and biases $b_1$, $b_2$ are shared across documents. Each document
%has its own parameters $\mu(X)$ and $\sigma(X)$ 
%resulting in a unique distribution $q(\theta | X)$ for each document. 
%The output of the encoder is a stochastic distributed representation of $X$ 
%denoted by $\theta$ which is a sample from $q(\theta | X)$. 
%$\theta$ depicts the semantic information encoded in the document $D$. 
%It can be interpreted as a topic proportion vector such as in classical topic modeling. \\\\
%% ======================================================================
%%  DECODER
%% ======================================================================
%\parhead{Decoder:}
%The decoder takes the sequential representation of the whole document (stop words included) 
%and predicts each word conditionally given all the preceding words using an RNN.
%Let $X^{\text{full}} \in R^{N_B \text{x} T}$ be the input document where $N_B$ is the number of sequences 
%of length $T$ in the document and $T$ is the number of unrolled steps of the RNN. 
%Each element of $X^{\text{full}}$ is a token from $0$ to $|V|$ where $|V|$ is the size of the vocabulary. 
%Denote by $\mathcal{S}$ the set of stop words. This set is pre-specified. Let $w_1, ..., w_T$ be 
%one sequence in $X^{\text{full}}$. To this sequence we associate $l_1, ..., l_T$ where 
%$l_t = I(w_t \in \mathcal{S})$ indicates whether $w_t$ is a stop word. 
%The decoder models the observations $w_1, ..., w_T$ and $l_1, ..., l_T$ as follows:
%\begin{align*}
%	p_{\phi}(w_1,...,w_T, l_1,...,l_T) &= \prod_{t=1}^{T} p_{\phi}(w_t | w_{1:t-1}, l_t, \theta)p_{\phi}(l_t)
%\end{align*}
%where $\phi$ denotes the parameters of the RNN. Define $h_t = g(w_t)$ where $g$ is an RNN cell. 
%\begin{align*}
%	p_{\phi}(l_t) &= \text{Bernoulli}(\sigma(\gamma^Th_t))
%\end{align*}
%The predictive distribution over the word $w_t$, $p_{\phi}(w_t | w_{1:t-1}, l_t, \theta)$ 
%is the mixture of two multinomials where 
%the mixing proportions are given by $p_{\phi}(l_t = 1)$ and $1 - p_{\phi}(l_t = 1)$. More specifically
%\begin{align*}
%	p_{\phi}(w_t | w_{1:t-1}, l_t, \theta)
%	&= \sigma(\gamma^Th_t) \cdot \text{softmax}(V^Th_t + b) + 
%		\sigma(-\gamma^Th_t) \cdot \text{softmax}(V^Th_t + b + B\theta w_t)
%\end{align*}
%where the weight matrices $V$ and $B$ and bias $b$ are parameters of the decoder and
%are illustrated in \Cref{fig:architecture}. $B$ is a real matrix that can still be interpreted as 
%the topic matrix in classical topic modeling. \\\\
%% ======================================================================
%%  LEARNING
%% ======================================================================
%\parhead{Learning:}
%The parameters of the encoder and decoder are jointly optimized to maximize the 
%marginal log likelihood of the observed words $X^{\text{full}}$ and stop word indicators $l^{\text{full}}$:
%\begin{align*}
%	\log p(X^{\text{full}}, l^{\text{full}}) &= \log \sum_{\theta}^{} p(X^{\text{full}}, l^{\text{full}} | \theta)p(\theta)
%\end{align*}
%where $p(\theta)$ is the prior distribution over $\theta$ and is chosen to be standard Gaussian 
%throughout our experiments. This marginal distribution is intractable. We borrow ideas 
%from neural variational inference~\citep{mnih2014neural} and maximize a lower bound on 
%the log marginal likelihood called the \gls{ELBO}: 
%\begin{align*}
%	\gls{ELBO} &= E_{q(\theta | X)}[\log p(X^{\text{full}}, l^{\text{full}} | \theta)] - 
%				\glsunset{KL}\gls{KL}(q(\theta | X) \gg p(\theta)) \\
%			&= \sum_{i=1}^{N_B} \sum_{t=1}^{T} \log p_{\phi}(w_{it} | w_{i_1:i_{t-1}}, l_{it}, \theta) + 
%				\log p(\theta) - \gls{KL}(q(\theta | X) \gg p(\theta))
%\end{align*}
%Given that both the prior $p(\theta)$ and the variational distribution $q(\theta | X)$ are 
%Gaussian, the \gls{KL} term can be written in an analytic closed-form:
%\begin{align*}
%	\gls{KL}(q(\theta | X) \gg p(\theta)) &= -\frac{1}{2} (K - \mu(X)^T\mu(X) - 
%		\sigma(X)^T\sigma(X) +\log |\diag(\sigma(x)^T\sigma(X))|)
%\end{align*}
%During training, the inference network and the model parameters 
%are jointly trained and updated via truncated back-propagation through time 
%using the Adam~\citep{kingma2014adam} algorithm and stochastic samples from $q(\theta|X)$.
%Using the reparameterization trick~\cite{rezende2014stochastic} and the analytic 
%form of the \gls{KL} term above yields unbiased and low variance gradients.
%\\\\
% ======================================================================
%   COMPLETE TEXT GENERATION ALGORITHM
% ======================================================================
\parhead{Generating sequential text and computing perplexity.}
Suppose we are given a word sequence $y_{1:t-1}$, from which we have
an initial estimation of $q(\theta | X_c)$. To generate the next word
$y_t$, we compute the probability distribution of $y_t$ given
$y_{1:t-1}$ in an online fashion. 
We %represent 
choose
$\theta$ to be a point estimate $\hat{\theta}$, the mean of its 
current distribution $q(\theta | X_c)$. 
Marginalizing over the 
stop word indicator $l_t$ which is unknown prior to 
observing $y_t$, the approximate distribution of $y_t$ is 
\begin{align*}
  p(y_t | y_{1:t-1}) \approx  \sum_{l_t} p(y_t |
  h_t,\hat{\theta}, l_t)p(l_t | h_t) .
\end{align*}
%After $y_t$ is observed we update $q(\theta | X_c)$ 
The predicted word $y_t$ is a sample from this predictive distribution.
We update $q(\theta | X_c)$ by including $y_t$ to $X_c$ if $y_t$ is 
not a stop word. However, updating $q(\theta| X_c)$ after each word
prediction is expensive, so we use a sliding window
as was done in~\citet{mikolov2012context}. To compute the perplexity, we 
use the approximate predictive distribution above.


%TopicRNN is a deep generative model of text. To generate text from it is straightforward. 
%There are two seeds that need to be provided: a document seed and a word seed. 
%The document seed is used to compute $\theta$ which will be used as bias to the output
%of the generator. This context vector $\theta$ is computed by sampling from
%the frozen inference network whose weights have been learned during training. 
%The seed word is passed through the frozen RNN decoder. 
%The hidden state of this RNN is conditioned upon to compute the probability of generating a stop word. 
%If this probability is beyond the threshold of $0.5$ then a stop word is generated by sampling
%from $\text{softmax}(V^Th_t + b)$ restraining this vector to the stop word set. 
%Otherwise a content word is generated by sampling from $\text{softmax}(V^Th_t + b + B\theta w_t)$
%truncated to exclude stop words. The new generated word is used as input and the procedure 
%is repeated to generate text.

%\iffalse
\parhead{Model Complexity.}
\acrlong{TopicRNN} has a complexity of 
$O(H\times H + H \times (C + K) + W_c)$,
where $H$ is the size of the hidden layer of the \acrshort{RNN},
$C$ is the vocabulary size, $K$ is the dimension of the 
topic vector, and $W_c$ is the number of parameters 
of the inference network. 
%\acrlong{TopicRNN} trades off 
%an extra $O(W_c)$ in complexity 
%as compared to 
The contextual 
\acrshort{RNN} of~\citet{mikolov2012context} 
accounts for $O(H\times H + H \times (C + K))$, not including the pre-training process, which
might require more parameters than the additional $W_c$ in our complexity. 
%with better performance across different 
%tasks (word prediction and sentiment analysis).
%The bottleneck -- as in most neural network-based 
%language models -- is in the output layer.
% There are many solutions for reducing this bottleneck: 
%factorization of the output layer,
%output layer compression, hierarchical softmax,
%and the most recent efficient softmax~\citep{grave2016efficient}.
%All these techniques are applicable to \acrlong{TopicRNN}.
%\fi

